Speaking in Words, Thinking in Logic: A Dual-Process Framework in QA Systems

Recent advances in large language models (LLMs) have significantly enhanced question-answering (QA) capabilities, particularly in open-domain contexts. However, in closed-domain scenarios such as education, healthcare, and law, users demand not only accurate answers but also transparent reasoning and explainable decision-making processes. While neural-symbolic (NeSy) frameworks have emerged as a promising solution, leveraging LLMs for natural language understanding and symbolic systems for formal reasoning, existing approaches often rely on large-scale models and exhibit inefficiencies in translating natural language into formal logic representations. To address these limitations, we introduce Text-JEPA (Text-based Joint-Embedding Predictive Architecture), a lightweight yet effective framework for converting natural language into first-order logic (NL2FOL). Drawing inspiration from dual-system cognitive theory, Text-JEPA emulates System 1 by efficiently generating logic representations, while the Z3 solver operates as System 2, enabling robust logical inference. To rigorously evaluate the NL2FOL-to-reasoning pipeline, we propose a comprehensive evaluation framework comprising three custom metrics: conversion score, reasoning score, and Spearman rho score, which collectively capture the quality of logical translation and its downstream impact on reasoning accuracy. Empirical results on domain-specific datasets demonstrate that Text-JEPA achieves competitive performance with significantly lower computational overhead compared to larger LLM-based systems. Our findings highlight the potential of structured, interpretable reasoning frameworks for building efficient and explainable QA systems in specialized domains.

==> figures_latex/result_pure_llm_folio/pure_llm_folio_FOL_CoT.tex <==
\begin{tikzpicture}
	\begin{axis}[
		width=10cm, height=10cm,
		%colormap={bluered}{rgb255(0cm)=(255,255,255); rgb255(1cm)=(0,56,168)}, % Giá trị lớn màu đậm
		colormap={tealwhite}{rgb255(0cm)=(255,255,255); rgb255(1cm)=(0,128,128)}, % Giá trị lớn màu t
		point meta min=0,
		point meta max=60,
		enlargelimits=false,
		scale only axis,
		tick label style={font=\small},
		ytick={0.25, 1, 2},
		yticklabels={True, False, Unknown},
		xtick={0.25, 1, 2},
		xticklabels={True, False, Unknown},
		axis on top,
		xlabel=Predicted,
		ylabel=Actual,
		nodes near coords,
		every node near coord/.append style={font=\bfseries\small, text=black}, % Định dạng Bold cho số
		]
		\addplot [matrix plot, mesh/cols=3, mesh/rows=3,
		point meta=explicit] 
		table [meta=C] {
			X Y C
			0 0 61
			1 0 7
			2 0 4
			0 1 23
			1 1 37
			2 1 3
			0 2 35
			1 2 15
			2 2 19
		};
	\end{axis}
\end{tikzpicture}


==> figures_latex/result_pure_llm_folio/pure_llm_folio_FOL_ZShot.tex <==
\begin{tikzpicture}
	\begin{axis}[
		width=10cm, height=10cm,
		%colormap={bluered}{rgb255(0cm)=(255,255,255); rgb255(1cm)=(0,56,168)}, % Giá trị lớn màu đậm
		colormap={tealwhite}{rgb255(0cm)=(255,255,255); rgb255(1cm)=(0,128,128)}, % Giá trị lớn màu t
		point meta min=0,
		point meta max=60,
		enlargelimits=false,
		scale only axis,
		tick label style={font=\small},
		ytick={0.25, 1, 2},
		yticklabels={True, False, Unknown},
		xtick={0.25, 1, 2},
		xticklabels={True, False, Unknown},
		axis on top,
		xlabel=Predicted,
		ylabel=Actual,
		nodes near coords,
		every node near coord/.append style={font=\bfseries\small, text=black}, % Định dạng Bold cho số
		]
		\addplot [matrix plot, mesh/cols=3, mesh/rows=3,
		point meta=explicit] 
		table [meta=C] {
			X Y C
			0 0 65
			1 0 0
			2 0 7
			0 1 30
			1 1 25
			2 1 8
			0 2 38
			1 2 10
			2 2 21
		};
	\end{axis}
\end{tikzpicture}


==> figures_latex/result_pure_llm_folio/pure_llm_folio_NL_CoT.tex <==
\begin{tikzpicture}
	\begin{axis}[
		width=10cm, height=10cm,
		%colormap={bluered}{rgb255(0cm)=(255,255,255); rgb255(1cm)=(0,56,168)}, % Giá trị lớn màu đậm
		colormap={tealwhite}{rgb255(0cm)=(255,255,255); rgb255(1cm)=(0,128,128)}, % Giá trị lớn màu t
		point meta min=0,
		point meta max=60,
		enlargelimits=false,
		scale only axis,
		tick label style={font=\small},
		ytick={0.25, 1, 2},
		yticklabels={True, False, Unknown},
		xtick={0.25, 1, 2},
		xticklabels={True, False, Unknown},
		axis on top,
		xlabel=Predicted,
		ylabel=Actual,
		nodes near coords,
		every node near coord/.append style={font=\bfseries\small, text=black}, % Định dạng Bold cho số
		]
		\addplot [matrix plot, mesh/cols=3, mesh/rows=3,
		point meta=explicit] 
		table [meta=C] {
			X Y C
			0 0 60
			1 0 7
			2 0 4
			0 1 18
			1 1 37
			2 1 7
			0 2 33
			1 2 22
			2 2 14
		};
	\end{axis}
\end{tikzpicture}


==> figures_latex/result_pure_llm_folio/pure_llm_folio_NL_ZShot.tex <==
\begin{tikzpicture}
	\begin{axis}[
		width=10cm, height=10cm,
		%colormap={bluered}{rgb255(0cm)=(255,255,255); rgb255(1cm)=(0,56,168)}, % Giá trị lớn màu đậm
		colormap={tealwhite}{rgb255(0cm)=(255,255,255); rgb255(1cm)=(0,128,128)}, % Giá trị lớn màu teal
		point meta min=0,
		point meta max=60,
		enlargelimits=false,
		scale only axis,
		tick label style={font=\small},
		ytick={0.25, 1, 2},
		yticklabels={True, False, Unknown},
		%xtick={0.5, 1.5, 2.5},
		xtick={0.25, 1, 2},
		xticklabels={True, False, Unknown},
		axis on top,
		xlabel=Predicted,
		ylabel=Actual,
		nodes near coords,
		every node near coord/.append style={font=\bfseries\small, text=black}, % Định dạng Bold cho số
		]
		\addplot [matrix plot, mesh/cols=3, mesh/rows=3,
		point meta=explicit] 
		table [meta=C] {
			X Y C
			0 0 62
			1 0 0
			2 0 10
			0 1 27
			1 1 27
			2 1 9
			0 2 36
			1 2 13
			2 2 20
		};
	\end{axis}
\end{tikzpicture}

